Edge: Enriching Knowledge Graph Embeddings with External Text

Knowledge graphs suffer from sparsity which degrades the quality of representations generated by various methods. While there is an abundance of textual information throughout the web and many existing knowledge bases, aligning information across these diverse data sources remains a challenge in the literature. Previous work has partially addressed this issue by enriching knowledge graph entities based on "hard" co-occurrence of words present in the entities of the knowledge graphs and external text, while we achieve "soft" augmentation by proposing a knowledge graph enrichment and embedding framework named Edge. Given an original knowledge graph, we first generate a rich but noisy augmented graph using external texts in semantic and structural level. To distill the relevant knowledge and suppress the introduced noise, we design a graph alignment term in a shared embedding space between the original graph and augmented graph. To enhance the embedding learning on the augmented graph, we further regularize the locality relationship of target entity based on negative sampling. Experimental results on four benchmark datasets demonstrate the robustness and effectiveness of Edge in link prediction and node classification.

==> tex/05-discussion.tex <==
% Next, we examine our model in more details and study how different parameters affect its performance\footnote{We plan to release our code upon publication.}.

% \subsection{Parameter Sensitivity}
% We evaluate the parameterization of EDGE, and specifically we examine how changes to our loss function hyper parameters, $\alpha$, $\beta$, and $\gamma$, could affect the model performance in the task of link prediction on Cora and Citeseer datasets. In each analysis we fix the values of two of the three parameters and study the effect of the variation of the third parameter on evaluating AUC scores across 200 epochs. In all experiments we used TF-IDF values as the input feature matrix. The result is illustrated in Figure \ref{fig:param}.

% Figures \ref{subfig:cora_beta1gamma1} and \ref{subfig:citeseer_beta1gamma1} show the effect of varying $\alpha$ when $\beta=1$ and $\gamma=1$ are fixed. We observe a somewhat consistent trend across performance for different values of $\alpha$. Decreasing $\alpha$ until $0.01$ improves the score but its further decline to $0.001$ does not raise the performance. $\alpha$ is the coefficient of $\mathcal{L}_T$ (see Equation \ref{eq:lt}) and this examination suggests that the effect of this loss function is less significant, because we re-address it in the $\mathcal{L}_N$ part of the loss function where we consider the same graph ($a\mathcal{KG}$) and try to optimize distance between its nodes but with more constraints.

% Figures \ref{subfig:cora_alpha1gamma1} and \ref{subfig:citeseer_alpha1gamma1} illustrate the effect of varying $\beta$ while $\alpha=1$ and $\gamma=1$ are fixed. Tuning $\beta$ results in more radical changes in the model performance which is again consistent between the two datasets. Small values for $\beta$ degrades performance remarkably, and we observe a much more improved AUC score for larger values of $\beta$. This implies the dominant effect of the joint loss function that is defined as the distance between corresponding entities of $\mathcal{KG}$ and $a\mathcal{KG}$, \ref{eq:lj}.

% Next, we fix $\alpha=1$ and $\beta=1$ and tweak $\gamma$ from $0.1$ to $10$. As Figures \ref{subfig:cora_alpha1beta1} and \ref{subfig:citeseer_alpha1beta1} reveal, the resulting graphs are not consistent with each other, but the variation in performance is small and in practice we obtain the results when $\gamma=1$ and $\beta=10$ for both Cora and Citeseer. In fact, the takeaway here is that the effect of $\mathcal{L}_J$ should be 10 times as the effect of $\mathcal{L}_N$. 

% Finally, as we obtained the best results when $\beta=10$, we set $\gamma=1$ and once again tune $\alpha$. Figures \ref{subfig:cora_beta10gamma1} and \ref{subfig:citeseer_beta10gamma1} show the results for this updated setting. These experiments reveal that $\beta$ should be $1000$ times larger than $\alpha$ which confirms the first observation and it is also consistent with the previous finding that $\beta$ should be $10$ times larger than $\gamma$.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=.63\columnwidth]{Figures/distance_cdf.pdf}
%     \caption{Distribution of pair-wise distance of entities for $\mathcal{KG}$ and $a\mathcal{KG}$ for SNOMED dataset.}
%     \label{fig:dist}
% \end{figure}



% % \subsection{Qualitative Analysis}
% % \label{subsec:QA}
% % Here we examine the process of textual graph generation. We find textual features for sample entities of our knowledge graph from an external text. Table \ref{tab:gt_gen} represents two sample entities from SNOMED knowledge graph. For both entities we list entities obtained from node2vec and doc2vec based on similarity in the second and the third columns, respectively. The top keywords from running LDA on top of all these entities are given in the fourth column, and entities extracted from running Stanford IE on WordNet sentences are shown in the last column. 

% % As it is clearly evident, both node2vec and doc2vec output very similar entities to the target entity. Note that the first target entity is in the list of node2vec top 4 most similar entities of the second target entity. The top query keywords for the two samples indicate that although they are very similar entities, their query keywords are not necessarily identical. In this case they share two and each has two distinct keywords. Finally, in the last column, we observe that new textual features are clearly different from our initial feature set and can definitely be used to enhance the initial knowledge graph. Besides, since the two target entities share two textual nodes, \textit{pathological state} and \textit{microorganism}, the distance between the two target entities decreases. 

% \subsection{Augmented KG Effectiveness}
% To show how pair-wise distance (length of the shortest path) among entities decreases in $a\mathcal{KG}$ we plot the distribution of all pair-wise distances for $\mathcal{KG}$ and $a\mathcal{KG}$ for SNOMED knowledge graph in Figure \ref{fig:dist}. As this figure depicts the pair-wise distance is evidently smaller in $a\mathcal{KG}$ which is the result of adding new textual nodes to the original knowledge graph. We conclude that the feature propagation operation in EDGE is more effective.


% Additionally, we claim that $a\mathcal{KG}$ provides complementary information, so that our approach can uncover underlying structure of the knowledge graph that is essential for link prediction. To justify this assumption, we visualize the similarity matrix of node embeddings for two scenarios on Cora dataset: 1) GAE on $\mathcal{KG}$ and 2) EDGE on $\mathcal{KG}$ and $a\mathcal{KG}$. The results are presented in Figure \ref{fig:sim}. In this heatmap elements are pair-wise similarity values sorted by different labels (7 classes). We can observe that the block-diagonal structure learned by our approach is clearer than that of GAE, indicating enhanced separability between different classes.

